BLAZE: Cross-Language and Cross-Project Bug Localization via Dynamic Chunking and Hard Example Learning

Software bugs require developers to exert significant effort to identify and resolve them, often consuming about one-third of their time. Bug localization, the process of pinpointing the exact source code files that need modification, is crucial in reducing this effort. Existing bug localization tools, typically reliant on deep learning techniques, face limitations in cross-project applicability and effectiveness in multi-language environments. Recent advancements with Large Language Models (LLMs) offer detailed representations for bug localization. However, they encounter challenges with limited context windows and mapping accuracy. To address these issues, we propose BLAZE, an approach that employs dynamic chunking and hard example learning. First, BLAZE dynamically segments source code to minimize continuity loss. Then, BLAZE fine-tunes a GPT-based model using challenging bug cases, in order to enhance cross-project and cross-language bug localization. To support the capability of BLAZE, we create the BEETLEBOX dataset, which comprises 26,321 bugs from 29 large and thriving open-source projects across five different programming languages (Java, C++, Python, Go, and JavaScript). Our evaluations of BLAZE on three benchmark datasets BEETLEBOX, SWE-Bench, and Ye et al. demonstrate substantial improvements compared to six state-of-the-art baselines. Specifically, BLAZE achieves up to an increase of 120% in Top 1 accuracy, 144% in Mean Average Precision (MAP), and 100% in Mean Reciprocal Rank (MRR). An extensive ablation study confirms the contributions of our pipeline components to the overall performance enhancement.

==> Background.tex <==
\section{Background}
\label{sec:background}
In this section, we describe terms related to the bug localization problem, which 
we use throughout our study.
\subsection{Bug Localization Tools}

Bug localization tools use bug reports to identify the responsible \scf for software bugs. A bug report includes title, description, version, and possibly code examples. To localize the bug, a bug localization tool retrieves all source code files from a repository at the relevant version. After that, it calculates the relevancy of each \scf with the bug report. A deep learning-based tool uses a neural network to estimate the relevance between the embeddings of source code files and bug reports. Finally, it ranks the \scf based on their relevancy.
% Bug localization tools commonly use data sources, such as bug reports to determine the responsible \scf. A bug report typically provides information about the unexpected behavior of software and how to reproduce it, including a bug ID, title, textual description, and version of the codebase where the bug exists. Additionally, a bug report may include an example of code, stack trace, or logs. 
% A bug localization tool retrieves all source code files from a repository at the relevant version to localize the bug. For example, if there are 100 \scf in a repository, the tool will estimate the relevance between the bug report and each of these 100 files. This relevance can be measured in several ways, such as by counting the number of words in common or comparing the embedding of both the bug report and the \scf. Once the relevance has been calculated, the tool scales the relevance of all files to compare their relevance. In some cases, metrics such as cosine distance already provide a scaled value, allowing the tool to skip this step. After scaling the relevance, the tool ranks the files based on relevance. A deep learning-based tool uses a neural network to estimate the relevance between the embeddings of source code files and bug reports. The neural network output provides a scaled relevance between the bug report and the source code file. The ranked list of files is the final output of a bug localization tool.
\subsection{Within project bug localization}

In within-project bug localization, supervised models are trained for individual projects. Two main approaches are lexical retrieval (e.g., BM25~\cite{bm25}, TF-IDF~\cite{tfidf}) and deep learning. Lexical tools are simple and fast in matching bug reports with source code files but struggle with vocabulary mismatches. Deep learning-based tools~\cite{Liang2019, Li2019, Xiao2019, Huo2021} use  Word2Vec~\cite{Mikolov2013} or GloVe-style~\cite{Pennington2014} embedding models for better semantic understanding, but the context remains an issue. Large Language Models (LLMs) offer context-aware embeddings and improve deep learning-based bug localization~\cite{Huang2022, Ciborowska2022}. While these deep-learning-based models outperform lexical ones, they're domain-specific and lose effectiveness when used in a new project. 

% Within project bug localization refers to the technique where a supervised bug localization model is trained for every project.  There are several approaches followed for within-project bug localization. However, the two major categories of approaches are lexical and deep learning-based approaches.\par
% Lexical retrieval models (e.g., BM25~\cite{bm25}, TF-IDF~\cite{tfidf}) are used in information retrieval-based bug localization tools to capture the match between bug reports and \scf. These tools are simple, effective, and fast and have been at the forefront of research on bug localization for several years. Many bug localization tools still employ these models today~\cite{Zhou2012, Wang2014, Murali2021, Razzaq2021}. However, one disadvantage of using these models is their inability to identify related \scf when there is a mismatch in the vocabulary between the bug report and the \scf.\par
% Deep learning-based bug localization tools~\cite{Liang2019, Li2019, Xiao2019, Huo2021} utilize the deep understanding of the word (or tokens) in bug reports/source code files to relate bug reports with source code files. These tools rely on Word2Vec~\cite{Mikolov2013} or GloVe-style~\cite{Pennington2014} embedding models. The significant advantage of employing these tools is that when two distinct words have the same meaning, their embedding will be nearly identical.\par
% Word2Vec and other embedding models have partially addressed the issue of vocabulary mismatch. Nonetheless, the models' representation is not context-sensitive, even though word meaning/representation depends on context. Large Language Models (LLMs) have proven useful in generating context-aware sequence embedding. As a result of their distinctive capability, they have been utilized in numerous deep learning-based bug localization tools~\cite{Huang2022, Ciborowska2022}. While deep learning-based models outperform lexical tools, their superiority is restricted to a specific domain. If the underlying domain changes, the representation learned by the model may fail to adapt, resulting in a significant decrease in performance.
\subsection{Cross project Bug Localization}
Prior studies have proposed different approaches for bug localization, but they commonly employ a supervised technique. Nonetheless, the insufficiency of labeled data for training supervised models presents a significant challenge when employing these models in industrial settings~\cite{Huo2021, Murali2021}. Furthermore, the models must be trained separately for each project before deployment, which raises concerns regarding maintainability and scalability. Cross-project bug localization aims to solve the problem. Cross-project bug localization means the deployment of a bug localization model in a project with no or minimal training in that particular project. If the bug localization model is deployed with no project-specific training, that will be called the zero-shot environment, and with minimal training, it will be called the few-shot environment.

==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\begin{figure}[tb!]
    \centering   
        \includegraphics[scale=0.035]{Figures/MAP_BY_Language.png}
    \caption{Performance of models by language in terms of MAP.}
    \label{fig:radar_chart}
\end{figure}
In Figure~\ref{fig:radar_chart}, we present the performance of the tools by language in terms of MAP. A common pattern among the tools is that they achieve their best performance in the Go language and worst performance in Python.
One possible reason that models perform their worst in Python is that among these five languages, Python is an indentation-based language. The control blocks of Python are separated by indentation. The problem is that the models use a tokenizer to convert text (source code, bug report) into vectors. Later, these vectors are fed into the model. In the tokenization step, the indentation of the code is lost.


\bz compared to TRANP-CNN. The result indicates that \bz outperforms TRANP-CNN in all but two settings. To investigate the possible reason performance drop of \bz, we conducted further analysis. We hypothesize that \bz prioritizes token-level similarity, which may hurt its performance if there are significant differences between the tokens of two projects in the few-shot settings.\par
To verify our hypothesis, first, we tokenize the bug report of each project. After tokenization, we create the token set and calculate the percentage of tokens available in the source and target project. The results are presented in Figure~\ref{fig:token_heatmap}. \par
In Figure~\ref{fig:token_heatmap}, the columns represent the source project, while the rows represent the target project. For instance, the first row and the second column is presenting the percentage of common tokens when AspectJ is the source project and HttpClient is the target project. Please note the relationship is not symmetric; for example, when HttpClient is the source project and AspectJ is the target project (third row, first column), the percentage of common tokens is different. Figure~\ref{fig:token_heatmap} shows that in the 16 settings, two of the least common token percentage is in the setting HttpClient $\rightarrow$ AspectJ and Lucene-solr $\rightarrow$ AspectJ setting. Previously, in Table~\ref{Table:few_shot_performance}, TRANP-CNN achieved better performance only in these two settings. The analysis indicates that when there is a low similarity between the source and target projects, transferring the knowledge gained from the source project to the target project becomes challenging, which is consistent with earlier research studies~\cite{Ruder2017, Brandt2021}. Moreover, in Table~\ref{table:data_stat}, we notice that Lucene-solr and the HttpClient have the lowest number of localized bugs. The dataset size can also limit the generalizability of the models trained on these two projects.


==> Tables/Dataset.tex <==
\begin{table}[tb!]
\centering
\caption{Dataset statistics.}
\begin{tabular}{l r r}
\toprule
\textbf{Project} & \textbf{\# Closed Bugs} & \textbf{\# Localized Bugs} \\ \midrule
AspectJ (A)         & 693                & 371                          \\ \midrule 
HttpClient (H)      & 746                & 63                           \\ \midrule
Jackrabbit (JR)       & 2,042              & 534                          \\ \midrule
Lucene-solr (L)     & 2,044              & 196                          \\ \midrule

JDT (J)         & 6,274                 & 587                          \\ \midrule 

SWT (S)         & 4,151                & 1,122                          \\ \midrule 

Eclipse Platform UI (E)         & 6,495                & 971                          \\ 


\bottomrule
\end{tabular}
\label{table:data_stat}
\end{table}

==> Tables/dataset_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[tb!]
\centering
\tbl{
\caption{Performance comparison between \bz trained on different datasets.}
\label{table:dataset ablation}
\begin{tabular}{@{}llllll@{}}
\toprule
\textbf{Tools} & \textbf{Top 1} & \textbf{Top 5} & \textbf{Top 10} & \textbf{MAP} & \textbf{MRR} \\ \midrule
\bz\textsubscript{\bbox} & 0.18           & 0.37           & 0.45            & 0.22         & 0.27         \\ \midrule
\bz\textsubscript{Ye et al.} & 0.14           & 0.32           & 0.44            & 0.2          & 0.23         \\ \bottomrule
\end{tabular}
}
\end{table}

==> Tables/few_shot_performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!tb]
\centering
\caption{Few shot performance of BLAZE.}
\begin{tabular}{c|c|c|c}
\toprule
\multicolumn{1}{|c|}{\textbf{Project Name}} & \textbf{Method} & \textbf{MAP} & \textbf{MRR} \\ \midrule
\multirow{4}{*}{H -\textgreater A}          & BLAZE           & 0.36         & 0.48         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.397        & 0.479        \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.27         & 0.36         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.20         & 0.27         \\ \midrule
\multirow{4}{*}{J -\textgreater A}          & BLAZE           & 0.32         & 0.41         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.29         & 0.36         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.22         & 0.35         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.20         & 0.27         \\ \midrule
\multirow{4}{*}{L -\textgreater A}          & BLAZE           & 0.44         & 0.53         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.46         & 0.55         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.22         & 0.35         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.20         & 0.27         \\ \midrule
\multirow{4}{*}{A-\textgreater H}           & BLAZE           & 0.31         & 0.42         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.26         & 0.38         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.19         & 0.28         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.16         & 0.26         \\ \midrule
\multirow{4}{*}{J-\textgreater{}H}          & BLAZE           & 0.35         & 0.48         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.3          & 0.42         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.22         & 0.32         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.16         & 0.28         \\ \midrule
\multirow{4}{*}{L-\textgreater{}H}          & BLAZE           & 0.35         & 0.49         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.29         & 0.42         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.19         & 0.29         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.13         & 0.25         \\ \midrule
\multirow{4}{*}{A-\textgreater J}           & BLAZE           & 0.40         & 0.48         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.38         & 0.47         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.27         & 0.29         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.27         & 0.28         \\ \midrule
\multirow{4}{*}{H-\textgreater{}J}          & BLAZE           & 0.35         & 0.44         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.33         & 0.42         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.29         & 0.30         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.26         & 0.27         \\ \midrule
\multirow{4}{*}{L-\textgreater{}J}          & BLAZE           & 0.39         & 0.46         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.35         & 0.44         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.21         & 0.27         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.23         & 0.29         \\ \midrule
\multirow{4}{*}{A-\textgreater{}L}          & BLAZE           & 0.37         & 0.46         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.29         & 0.41         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.26         & 0.36         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.23         & 0.32         \\ \midrule
\multirow{4}{*}{H-\textgreater{}L}          & BLAZE           & 0.33         & 0.46         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.29         & 0.41         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.28         & 0.38         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.24         & 0.35         \\ \midrule
\multirow{4}{*}{J-\textgreater{}L}          & BLAZE           & 0.35         & 0.47         \\ \cmidrule{2-4} 
                                            & TRANP-CNN       & 0.26         & 0.39         \\ \cmidrule{2-4} 
                                            & DNNLoc          & 0.28         & 0.38         \\ \cmidrule{2-4} 
                                            & BugLocator      & 0.24         & 0.35         \\ \bottomrule
\end{tabular}
\label{Table:few_shot_performance}
\end{table}

==> Tables/few_shot_performance_cooba.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!tb]
\centering
\caption{Few shot performance of BLAZE in comparison to CooBa.}
\begin{tabular}{l l r l l r}
\toprule
\textbf{Project}              & \textbf{Method} & \textbf{MAP} & \textbf{Project}              & \textbf{Method} & \textbf{MAP} \\ \midrule
\multirow{2}{*}{A$\rightarrow$J} & BLAZE           & 0.40         & \multirow{2}{*}{A$\rightarrow$S} & BLAZE           & 0.33         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.31         &                                    & CooBA           & 0.28         \\ \midrule
\multirow{2}{*}{S$\rightarrow$J} & BLAZE           & 0.36         & \multirow{2}{*}{J$\rightarrow$S} & BLAZE           & 0.34         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.32         &                                    & CooBA           & 0.30          \\ \midrule
\multirow{2}{*}{E$\rightarrow$J} & BLAZE           & 0.37         & \multirow{2}{*}{E$\rightarrow$S} & BLAZE           & 0.31         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.35         &                                    & CooBA           & 0.26         \\ \midrule
\multirow{2}{*}{J$\rightarrow$A} & BLAZE           & 0.32         & \multirow{2}{*}{A$\rightarrow$E} & BLAZE           & 0.37         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.30         &                                    & CooBA           & 0.33         \\ \midrule
\multirow{2}{*}{S$\rightarrow$A} & BLAZE           & 0.30         & \multirow{2}{*}{J$\rightarrow$E} & BLAZE           & 0.36         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.26         &                                    & CooBA           & 0.30          \\ \midrule
\multirow{2}{*}{E$\rightarrow$A} & BLAZE           & 0.27         & \multirow{2}{*}{S$\rightarrow$E} & BLAZE           & 0.37         \\ \cmidrule{2-3} \cmidrule{5-6} 
                                   & CooBA           & 0.26         &                                    & CooBA           & 0.32         \\ \bottomrule
\end{tabular}
\label{Table:few_shot_cooba_performance}
\end{table}

==> Tables/few_shot_performance_double.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!tb]
\centering
\caption{Few shot performance of BLAZE in comparison to TRANP-CNN.}
\begin{tabular}{l l r r r r r l l r r r r r}
\toprule
\textbf{Project}                             & \textbf{Method}    & \textbf{Top 1} & \textbf{Top 5} & \textbf{Top 10} & \textbf{MAP}  & \textbf{MRR}  & \textbf{Project}                            & \textbf{Method}    & \textbf{Top 1} & \textbf{Top 5} & \textbf{Top 10} & \textbf{MAP}  & \textbf{MRR}  \\ \midrule
\multirow{2}{*}{H $\rightarrow$ A}  & BLAZE     & 0.33  & 0.60  & 0.74   & 0.36 & 0.48 & \multirow{2}{*}{A$\rightarrow$ JR} & BLAZE     & 0.38  & 0.57  & 0.60   & 0.40 & 0.48 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.35  & 0.58  & 0.69   & 0.39 & 0.47 &                                    & TRANP-CNN & 0.34  & 0.51  & 0.59   & 0.38 & 0.47 \\ \midrule
\multirow{2}{*}{JR $\rightarrow$ A} & BLAZE     & 0.20  & 0.45  & 0.65   & 0.32 & 0.41 & \multirow{2}{*}{H$\rightarrow$JR}  & BLAZE     & 0.29  & 0.52  & 0.60   & 0.35 & 0.44 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.17  & 0.43  & 0.59   & 0.29 & 0.36 &                                    & TRANP-CNN & 0.27  & 0.47  & 0.58   & 0.33 & 0.42 \\ \midrule
\multirow{2}{*}{L $\rightarrow$ A}  & BLAZE     & 0.41  & 0.61  & 0.70   & 0.44 & 0.53 & \multirow{2}{*}{L$\rightarrow$JR}  & BLAZE     & 0.32  & 0.49  & 0.59   & 0.39 & 0.46 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.44  & 0.65  & 0.73   & 0.46 & 0.55 &                                    & TRANP-CNN & 0.25  & 0.46  & 0.56   & 0.35 & 0.44 \\ \midrule
\multirow{2}{*}{A$\rightarrow$ H}   & BLAZE     & 0.32  & 0.54  & 0.61   & 0.31 & 0.42 & \multirow{2}{*}{A$\rightarrow$L}   & BLAZE     & 0.35  & 0.56  & 0.63   & 0.37 & 0.46 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.26  & 0.49  & 0.58   & 0.26 & 0.38 &                                    & TRANP-CNN & 0.29  & 0.49  & 0.59   & 0.29 & 0.41 \\ \midrule
\multirow{2}{*}{JR$\rightarrow$H}   & BLAZE     & 0.40  & 0.56  & 0.7    & 0.35 & 0.48 & \multirow{2}{*}{H$\rightarrow$L}   & BLAZE     & 0.34  & 0.57  & 0.63   & 0.33 & 0.46 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.32  & 0.52  & 0.62   & 0.30 & 0.42 &                                    & TRANP-CNN & 0.30  & 0.54  & 0.59   & 0.29 & 0.41 \\ \midrule
\multirow{2}{*}{L$\rightarrow$H}    & BLAZE     & 0.33  & 0.60  & 0.61   & 0.35 & 0.49 & \multirow{2}{*}{JR$\rightarrow$L}  & BLAZE     & 0.29  & 0.54  & 0.63   & 0.35 & 0.47 \\ \cmidrule{2-7} \cmidrule{9-14} 
                                    & TRANP-CNN & 0.30  & 0.54  & 0.59   & 0.29 & 0.42 &                                    & TRANP-CNN & 0.25  & 0.48  & 0.59   & 0.26 & 0.39 \\ \bottomrule
\end{tabular}
\label{Table:few_shot_performance}
\end{table*}

==> Tables/freeze_impact.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
 \aboverulesep=0ex
 \belowrulesep=0ex
\begin{table}[!tb]
\centering
\caption{Impact of layer freezing.}
\begin{tabular}{p{0.9cm} p{0.21cm}p{0.21cm}p{0.21cm}p{0.38cm}p{0.2cm}p{0.2cm}p{0.2cm}p{0.34cm}}
\toprule
\multirow{2}{=}{\textbf{Project}} & \multicolumn{4}{c}{\textbf{MAP}}                                                                                            & \multicolumn{4}{c}{\textbf{MRR}}                                                                                             \\ \cmidrule(l{2pt}r{2pt}){2-5} \cmidrule(l{2pt}r{2pt}){6-9}  
                                       & \multicolumn{1}{c}{\textbf{30\%}} & \multicolumn{1}{c}{\textbf{50\%}} & \multicolumn{1}{c}{\textbf{70\%}} & \textbf{90\%} & \multicolumn{1}{c}{\textbf{30\%}} & \multicolumn{1}{c}{\textbf{50\%}} & \multicolumn{1}{c}{\textbf{70\%}} & \textbf{90\%} \\  \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
H$\rightarrow$ A                      & \multicolumn{1}{c}{0.37}          & \multicolumn{1}{c}{0.36}          & \multicolumn{1}{c}{0.34}          & 0.29          & \multicolumn{1}{c}{0.46}          & \multicolumn{1}{c}{0.48}          & \multicolumn{1}{c}{0.46}          & 0.42          \\  \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
JR$\rightarrow$ A                      & \multicolumn{1}{c}{0.31}          & \multicolumn{1}{c}{0.32}          & \multicolumn{1}{c}{0.3}           & 0.26          & \multicolumn{1}{c}{0.41}          & \multicolumn{1}{c}{0.41}          & \multicolumn{1}{c}{0.4}           & 0.39          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
L$\rightarrow$ A                      & \multicolumn{1}{c}{0.44}          & \multicolumn{1}{c}{0.44}          & \multicolumn{1}{c}{0.43}          & 0.40           & \multicolumn{1}{c}{0.50}          & \multicolumn{1}{c}{0.53}          & \multicolumn{1}{c}{0.51}          & 0.49          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
A$\rightarrow$H                       & \multicolumn{1}{c}{0.33}          & \multicolumn{1}{c}{0.31}          & \multicolumn{1}{c}{0.28}          & 0.26          & \multicolumn{1}{c}{0.42}          & \multicolumn{1}{c}{0.42}          & \multicolumn{1}{c}{0.4}           & 0.37          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
JR$\rightarrow$H                      & \multicolumn{1}{c}{0.31}          & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.32}          & 0.32          & \multicolumn{1}{c}{0.45}          & \multicolumn{1}{c}{0.48}          & \multicolumn{1}{c}{0.46}          & 0.45          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
L$\rightarrow$H                      & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.33}          & 0.31          & \multicolumn{1}{c}{0.48}          & \multicolumn{1}{c}{0.49}          & \multicolumn{1}{c}{0.47}          & 0.42          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
A$\rightarrow$JR                       & \multicolumn{1}{c}{0.40}           & \multicolumn{1}{c}{0.40}           & \multicolumn{1}{c}{0.37}          & 0.36          & \multicolumn{1}{c}{0.48}          & \multicolumn{1}{c}{0.48}          & \multicolumn{1}{c}{0.45}          & 0.45          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
H$\rightarrow$JR                      & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.33}          & 0.28          & \multicolumn{1}{c}{0.44}          & \multicolumn{1}{c}{0.44}          & \multicolumn{1}{c}{0.42}          & 0.42          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
L$\rightarrow$JR                      & \multicolumn{1}{c}{0.34}          & \multicolumn{1}{c}{0.39}          & \multicolumn{1}{c}{0.37}          & 0.33          & \multicolumn{1}{c}{0.47}          & \multicolumn{1}{c}{0.46}          & \multicolumn{1}{c}{0.43}          & 0.43          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
A$\rightarrow$L                      & \multicolumn{1}{c}{0.37}          & \multicolumn{1}{c}{0.37}          & \multicolumn{1}{c}{0.36}          & 0.31          & \multicolumn{1}{c}{0.46}          & \multicolumn{1}{c}{0.46}          & \multicolumn{1}{c}{0.43}          & 0.44          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
H$\rightarrow$L                      & \multicolumn{1}{c}{0.33}          & \multicolumn{1}{c}{0.33}          & \multicolumn{1}{c}{0.3}           & 0.25          & \multicolumn{1}{c}{0.40}          & \multicolumn{1}{c}{0.46}          & \multicolumn{1}{c}{0.43}          & 0.42          \\ \cmidrule(l{2pt}r{2pt}l{2pt}r{2pt}){1-9} 
JR$\rightarrow$L                      & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.35}          & \multicolumn{1}{c}{0.33}          & 0.31          & \multicolumn{1}{c}{0.44}          & \multicolumn{1}{c}{0.47}          & \multicolumn{1}{c}{0.46}          & 0.40           \\ \bottomrule
\end{tabular}
\label{table:layer_freeze}
\end{table}

==> Tables/result_ablation.tex <==
\begin{table}[!tb]
\caption{Performance of BLAZE using different components.}
\label{table:ablation_study}
\begin{tabular}{p{2.8cm}rrrrr}
\hline
\textbf{Variant}                & \textbf{Top 1} & \textbf{Top 5} & \textbf{Top 10} & \textbf{MAP} & \textbf{MRR} \\ \hline
Only ES                         & 0.10           & 0.23           & 0.41            & 0.21         & 0.26         \\
Only BugBERT      & 0.17           & 0.34           & 0.40            & 0.23         & 0.27         \\ \hline
Sliding Window  + BugBERT       & 0.29           & 0.58           & 0.61            & 0.29         & 0.38         \\
Static Chunking  + BugBERT      & 0.19           & 0.44           & 0.51            & 0.26         & 0.35         \\
Dynamic Chunking + BugBERT      & 0.30           & 0.60           & 0.63            & 0.31         & 0.40         \\ \hline
ES + Sliding Window  + BugBERT  & 0.30           & 0.61           & 0.67            & 0.31         & 0.40         \\
ES + Static Chunking  + BugBERT & 0.20           & 0.45           & 0.53            & 0.29         & 0.37         \\
ES + Dynamic Chunking + BugBERT & 0.31           & 0.68           & 0.74            & 0.34         & 0.44         \\ \hline
\end{tabular}
\end{table}
